Single-Image HDR Reconstruction by Learning to Reverse the Camera Pipeline

Recovering a high dynamic range (HDR) image from a single low dynamic range (LDR) input image is challenging due to missing details in under-/over-exposed regions caused by quantization and saturation of camera sensors. In contrast to existing learning-based methods, our core idea is to incorporate the domain knowledge of the LDR image formation pipeline into our model. We model the HDRto-LDR image formation pipeline as the (1) dynamic range clipping, (2) non-linear mapping from a camera response function, and (3) quantization. We then propose to learn three specialized CNNs to reverse these steps. By decomposing the problem into specific sub-tasks, we impose effective physical constraints to facilitate the training of individual sub-networks. Finally, we jointly fine-tune the entire model end-to-end to reduce error accumulation. With extensive quantitative and qualitative experiments on diverse image datasets, we demonstrate that the proposed method performs favorably against state-of-the-art single-image HDR reconstruction algorithms.

==> backup_1_introduction.tex <==

\section{Introduction}
\label{sec:intro}

HDR images are capable of capturing rich real-world scene appearances including lighting, contrast, and details.
Consumer-grade digital cameras, however, can only capture images within a limited dynamic range due to sensor constraints.
The most common approach to generate HDR images is to merge multiple LDR images captured with different exposures~\cite{debevec1997recovering}.
Such a technique performs well on static scenes but often suffers from ghosting artifacts on dynamic scenes or hand-held cameras.
Furthermore, capturing multiple images of the same scene may not always be feasible (e.g., existing LDR images on the Internet).

Single-image HDR reconstruction aims to recover an HDR image from a single LDR input.
The problem is challenging due to the missing information in under-/over-exposed regions.
Recently, several methods~\cite{marnerides2018expandnet,yang-cvpr18-DRHT,zhang2017learning} have been developed to reconstruct an HDR image from a given LDR input using deep convolutional neural networks (CNNs).
However, learning a direct LDR-to-HDR mapping is extremely difficult as the variation of HDR pixels (32-bit) is significantly higher than that of LDR pixels (8-bit).
Eilertsen~\etal~\cite{eilertsen2017hdrcnn} focus on recovering the over-exposed regions but ignore other artifacts caused by quantization and an inaccurate camera response function (CRF).
Endo~\etal~\cite{endo2017drtmo} propose an indirect approach by learning to synthesize several up-/down-exposed LDR images and then adopting the classic multi-image HDR reconstruction algorithm~\cite{debevec1997recovering} to obtain an HDR image. 
Nevertheless, it remains challenging to predict LDR images with different exposures due to the non-linear CRF in the camera pipeline.

In this work, we incorporate the domain knowledge of the LDR image formation pipeline to design our model.
We model the formation of an LDR image from an HDR image with the following steps~\cite{debevec1997recovering}: (1) dynamic range clipping, (2) non-linear mapping with a CRF, and (3) quantization.
Instead of learning a direct LDR-to-HDR mapping using a generic network, our core idea is to decompose the single-image HDR reconstruction problem into three sub-tasks: i) dequantization, ii) linearization, and iii) hallucination, and develop three deep networks to specifically tackle each of the tasks.
First, given an input LDR image, we apply a Dequantization-Net to restore the missing details caused by quantization and reduce the visual artifacts in the under-exposed regions (e.g., banding artifacts).
Second, we estimate an inverse CRF with a Linearization-Net and convert the non-linear LDR image to a \emph{linear} image (i.e., scene irradiance).
Building upon the empirical model of responses for CRFs~\cite{grossberg2003space}, our Linearization-Net leverages the additional cues from edge and intensity histogram and a monotonically increasing constraint to estimate more accurate CRFs.
Third, we predict the missing content in the over-exposed regions with a Hallucination-Net.
Finally, we jointly fine-tune the whole model to reduce error accumulation and boost overall performance.

The proposed networks explicitly model the \emph{inverse} functions of the LDR image formation pipeline.
By integrating the domain knowledge with deep CNNs, we significantly reduce the difficulty of training one single network for reconstructing HDR images.
To improve the robustness and generalization of our model, we introduce realistic Poisson-Gaussian noise~\cite{foi2008practical} when synthesizing the LDR images for training.
We evaluate the effectiveness of our method on a large-scale HDR image dataset, a RAW-jpeg dataset~\cite{dang2015raise}, as well as real-world LDR images captured from different cameras.
Extensive quantitative and qualitative evaluations, as well as the user study, demonstrate that our model performs favorably against the state-of-the-art single-image HDR reconstruction algorithms.
\figref{teaser} shows that the proposed method recovers visually pleasing results with faithful details.
Our contributions in this work are three-fold:
\begin{compactitem}
\item We model the single-image HDR reconstruction problem as an inverse LDR image formation pipeline, including the dequantization, linearization, and hallucination, and train three deep CNNs to address these sub-tasks accordingly.
\item We introduce specific physical constraints, input features, and loss functions for training each individual network and demonstrate the effectiveness of the proposed model over other alternatives.
\item We collect two HDR image datasets, one with synthetic LDR images and the other with real LDR images, for training and evaluation.
We demonstrate that the proposed method performs favorably against the state-of-the-art approaches in terms of the HDR-VDP-2 scores and visual quality.
\end{compactitem}


==> backup_3_method.tex <==

\section{Learning to Reverse the Camera Pipeline}
\label{sec:algorithm}

In this section, we first introduce the image formation pipeline that renders an LDR image (a regular image) from an HDR image (the scene irradiance) as shown in \figref{pipeline}(a).
We then describe the design methodology and training procedures of the proposed Dequantization-Net, Linearization-Net, and Hallucination-Net for reconstructing an HDR image from an LDR image by reversing the image formation pipeline as depicted in \figref{pipeline}(e).


\subsection{LDR image formation}
\label{sec:formation}
While the real scene irradiance has a high dynamic range, the digital sensor in cameras can only capture and store a limited extent, usually with 8 bits.
Given the irradiance $\irradiance$ and sensor exposure time $\exposure$, an HDR image is recorded by $\hdr = \irradiance \times \exposure$.
The process of converting one HDR image to one LDR image can be modeled by the following major steps:

\vspace{1mm}
\noindent{(1) \textbf{Dynamic range clipping}.}
The camera first clips the pixel values of an HDR image $\hdr$ to a limited range, which can be formulated by $\cliphdr = \clipping{\hdr} = \min{(\hdr, 1)}$.
Due to the clipping operation, there is information loss for pixels in the over-exposed regions. 

\vspace{1mm}
\noindent{(2) \textbf{Non-linear mapping}.}
To match the human perception of the scene, a camera typically applies a non-linear CRF mapping to adjust the contrast of the captured image.
One CRF maps a linear image to a non-linear image $\nonlinearhdr =  \crfmapping{\cliphdr}$.
A CRF is unique to the camera model and unknown in our problem setting.

\vspace{1mm}
\noindent{(3) \textbf{Quantization}.}
After the non-linear mapping, the recorded pixel values are quantized to 8 bits by 
$\quantizing{\nonlinearhdr} = \left \lfloor 255 \times \nonlinearhdr + 0.5 \right \rfloor / 255$. 
The quantization process leads to errors in the under-exposed and smooth gradient regions.

Taking all three steps into account, an LDR image $\ldr$ is formed by:
\begin{equation} \label{eq:pipeline}
    \ldr = \applypipeline{\hdr} = \quantizing{\crfmapping{\clipping{\hdr}}}\,,
\end{equation}
where $\pipeline$ is a function that integrates the dynamic range clipping, non-linear mapping, and quantization steps. 
The HDR reconstruction process aims to obtain the inverse function of $\pipeline$ to convert an LDR image to an HDR image.

To learn the inverse mapping $\invpipeline$, we propose to decompose the HDR reconstruction task into three sub-tasks: dequantization, linearization, and hallucination, which model the inverse functions of the quantization, non-linear mapping, and dynamic range clipping, respectively.
We train three CNNs for the three sub-tasks using the corresponding supervisory signal and specific physical constraints.
These three networks can be integrated into an end-to-end model and jointly fine-tuned to further reduce error accumulation and improve the performance.

\subsection{Dequantization}
Quantization often results in scattered noise or contouring artifacts in smooth regions (see \figref{vis_deq}(a)).
Therefore, we train a Dequantization-Net to reduce the quantization artifacts in the input LDR image.

\heading{Architecture.}
Our Dequantization-Net adopts a U-Net architecture, which is composed of an encoder and a decoder, with skip connections and 6 hierarchies.
Each hierarchy consists of two convolution layers followed by Leaky ReLU ($\alpha = 0.1$) layers.
We use the \texttt{Tanh} layer to normalize the output of the last layer to $[-1.0, 1.0]$.
Finally, we add the output of the Dequantization-Net with the input LDR image to produce the dequantized LDR image $\deqout$.

\heading{Training.}
We minimize the $\ltwo$ loss between the dequantized LDR $\deqout$ image and corresponding ground-truth image $\nonlinearhdr$:
\begin{align} \label{eq:deq_loss}
    \deqloss = \normtwo{\deqout - \nonlinearhdr} \,.
\end{align}
We note that $\nonlinearhdr = \crfmapping{\clipping{\hdr}}$ is constructed from the ground-truth HDR image with dynamic range clipping and non-linear mapping.

\heading{Discussion.}
The method of Liu~\etal~\cite{liu2018learning} aims at low-light image enhancement and uses a generative adversarial network~\cite{goodfellow2014generative} to restore realistic details.
However, we find that the adversarial loss often introduces noise-like details and does not improve the visual quality and performance of the Dequantization-Net.
Thus, we do not use the adversarial loss in our training.

\subsection{Linearization}
The goal of linearization (i.e., radiometric calibration) is to estimate a CRF and convert a non-linear LDR image to a linear irradiance.
Although the CRF (denoted by $\crf$) is distinct for each camera device, all the CRFs must have the following properties.
First, the function should be monotonically increasing.
Second, the minimal and maximal input values should be respectively mapped to the minimal and maximal output values: $\crfmapping{0} = 0$ and $\crfmapping{1} = 1$ in our case.
As the CRF is a one-to-one mapping function, the inverse CRF (denoted by $\invcrf = \crf^{-1}$) also has the above properties.

To represent a CRF, we first discretize an inverse CRF by uniformly sampling 1024 points between $[0, 1]$.
Therefore, an inverse CRF is represented as a 1024-dimensional vector $\invcrfvector \in \mathbb{R}^{1024}$.
We then adopt the Empirical Model of Response (EMoR) model~\cite{grossberg2003space}, which assumes that each inverse CRF $\invcrfvector$ can be approximated by a linear combination of $K$ PCA basis vectors $\invcrfvector_k$:
\begin{align} \label{eq:pca}
    \invcrfvector = \invcrfvector_0 + \sum_{k=1}^{K} \pcaweight_k \invcrfvector_k \,,
\end{align}
where $\invcrfvector_0$ is the mean inverse CRFs in the database~\cite{grossberg2003space}.
In this work, we use $K = 11$ basis vectors as it has been shown to capture the variations well in the CRF dataset~\cite{li2017crfnet}.
To predict the inverse CRF, we train a Linearization-Net to estimate the weights $\pcaweight_k$ from the input non-linear LDR image.

\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{imgs/method/histogram_1D.pdf}
    \figmargin
    \caption{
        \textbf{Proposed spatial-aware soft histogram layer.}
        We extract histogram features by a soft counting on pixel intensities and preserve the spatial information.
    }
    \label{fig:histogram_feature}
\end{figure}


\heading{Input features.}
As the edge and color histogram have been shown effective to estimate an inverse CRF in conventional methods~\cite{lin2004radiometric,lin2005determining}, we first extract the edge and histogram features from the non-linear LDR image.
We adopt the Sobel filter to obtain the edge responses, resulting in 6 feature maps (two directions $\times$ three color channels).
To extract the histogram features, we propose a spatial-aware soft-histogram layer.
Specifically, given the number of histogram bins $B$, we construct a \emph{soft} counting of pixel intensities by:
\begin{align} \label{eq:histogram_layer}
    h(i,j,c,b) = 
    \begin{cases}
        1 - d \cdot B\,, & \text{if}~ d < \frac{1}{B} \\
        0\,, & \text{otherwise}
    \end{cases}
\end{align}
where $i, j$ indicate horizontal and vertical pixel positions, $c$ represents the index for RGB color channels, $b \in \{1,\cdots, B\}$ is the index for the histogram bin, and $d = | I(i,j,c) - (2b - 1) / (2B) |$ is the intensity distance to the center of the $b$-th bin.
We note that the range of input pixel intensity is within $[0, 1]$.
Thus, $1 / B$ is the width of a bin. 
Every pixel contributes to the two nearby bins according to the intensity distance to the center of each bin.
Our histogram feature can be considered as the probability that a pixel $I(i, j, c)$ belongs to a bin $b$.
\figref{histogram_feature} shows a 1D example of our soft-histogram layer.


Our histogram layer preserves the spatial information and is fully differentiable.
We compute the histogram features for each RGB channel and concatenate the features together, thereby obtaining a total of $3B$ channels of histogram features.
In addition, we compute histogram features for $B = 4, 8, 16$ to capture information from different resolutions of the histogram bins.
As a result, we obtain a total $84 = 3 \cdot (4 + 8 + 16)$ histogram maps.
Along with the input non-linear image (3 channels) and edge responses (6 channels), the input to the Linearization-Net is a 93-channel feature.


\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/method/linearization_net.pdf}
    \caption{
        \textbf{Architecture of the Linearization-Net.}
        Given a non-linear LDR image, we first use the Sobel filter to compute gradient maps and extract histogram features using the proposed soft histogram layer.
        Our Linearization-Net then takes as input the non-linear LDR image, edge maps, and histogram maps, and predicts the PCA coefficients for reconstructing an inverse CRF from~\eqnref{pca}.
        To ensure that the estimated inverse CRF is monotonically increasing, we adjust the inverse CRF by subtracting the minimal first-order derivative (if negative) and normalizing the range to $[0, 1]$.
    }
    \label{fig:lin_net}
\end{figure*}


\heading{Architecture.}
We use the architecture of the ResNet-18~\cite{he2016deep} as the backbone of our Linearization-Net.
To extract a global feature and handle arbitrary image resolutions, we add a global average pooling layer after the last convolutional layer.
We then use two fully-connected layers to generate $K$ PCA weights and reconstruct an inverse CRF from~\eqnref{pca}.

\heading{Monotonically increasing constraint.}
To satisfy the constraint that a CRF/inverse CRF should be monotonically increasing, we adjust the estimated inverse CRF by enforcing all the first-order derivatives to be non-negative.
Specifically, we calculate the first-order derivatives by $\invcrfder_1 = 0$ and $\invcrfder_d = \invcrfscalar_d - \invcrfscalar_{d-1}$ for $d \in [2, \cdots, 1024]$ and find the smallest negative derivative $\invcrfder_m = \min(\min_d(\invcrfder_d), 0)$.
We then shift the derivatives by $\norminvcrfder_d = \invcrfder_d - \invcrfder_m$.
The inverse CRF $\norminvcrfvector = [\norminvcrfscalar_1, \cdots,  \norminvcrfscalar_{1024}]$ is then reconstructed by integration and normalization:
\begin{align} \label{eq:crf_normalization}
    \norminvcrfscalar_d = \frac{1}{ \sum_{i=1}^{1024} \norminvcrfder_i } \sum_{i=1}^{d} \norminvcrfder_i \,.
\end{align}
We normalize $\norminvcrfscalar_d$ by the summation of all derivatives to ensure the inverse CRF satisfies the constraint that $\invcrfmapping{0} = 0$ and $\invcrfmapping{1} = 1$.
\figref{lin_net} depicts the pipeline of our Linearization-Net. 
With the normalized inverse CRF $\norminvcrfvector$, we then map the non-linear LDR image $\deqout$ to a linear LDR image $\linout$.


\heading{Training.}
We define the linear LDR image reconstruction loss by:
\begin{align} \label{eq:lin_loss}
    \linloss = \normtwo{ \linout - \cliphdr} \,,
\end{align}
where $\cliphdr = \clipping{\hdr}$ is constructed from the ground-truth HDR image with the dynamic range clipping process.
In addition, we formulate the inverse CRF reconstruction loss by:
\begin{align}
    \crfloss = \normtwo{\norminvcrfvector - \invcrfvector} \,, 
\end{align}
where $\invcrfvector$ is the ground-truth inverse CRF.
We train the Linearization-Net by optimizing $\linloss + \crflossweight \crfloss$.
We empirically set $\crflossweight = 0.1$ in our experiments.



\heading{Discussion.}
The CRF-Net~\cite{li2017crfnet} also uses the ResNet-18 and EMoR model~\eqnref{pca} to estimate a CRF from the input non-linear LDR image.
However, the reconstructed CRF is not guaranteed to be monotonically increasing.
Moreover, the CRF-Net only operates on a fixed input resolution (e.g., $227 \times 227$).
When applying to images with a larger resolution, the CRF-Net selects 10 local patches and computes the average of the estimated CRFs from these patches.
In contrast, the proposed Linearization-Net uses a global pooling layer to handle arbitrary input resolutions and estimates an inverse CRF in a single feed-forward pass.
While we use additional input features and apply a monotonically increasing constraint to normalize the estimated inverse CRF, these operations only entail low computational load.
For an image with a resolution of $227 \times 227$ pixels, both the CRF-Net and our Linearization-Net can be executed efficiently (0.021 and 0.026 seconds, respectively).
For an image with a resolution of $512 \times 512$ pixels, the CRF-Net takes 5.1 seconds (0.212 seconds for PCA weights prediction on a GPU and 4.888 seconds for patch search on CPU), while our Linearization-Net takes 0.1 seconds on the same GPU.
We show more comparisons with alternative approaches and the CRF-Net in~\secref{ablation}.


\subsection{Hallucination}
After the dequantization and linearization processes, the last step is to recover the missing contents due to dynamic range clipping.
To this end, we train a Hallucination-Net (denoted by $\halnet{\cdot}$) to predict the missing details within the over-exposed regions.

\heading{Architecture.}
We adopt an encoder-decoder architecture with skip connections~\cite{eilertsen2017hdrcnn} as our Hallucination-Net.
The reconstructed HDR image is modeled by $\halout = \linout + \mask \cdot \halnet{\linout}$, 
where $\linout$ is the image generated from the Linearization-Net and $\mask = \max(0, \linout - \gamma) / (1 - \gamma)$ is the over-exposed mask with $\gamma = 0.95$.
Since the missing values in the over-exposed regions should always be greater than the existing pixel values, we constrain the Hallucination-Net to predict \emph{positive residuals} by adding a \texttt{ReLU} layer at the end of the network.
We note that our over-exposed mask is a \emph{soft} mask where $\mask \in [0, 1]$.
The mask value $\mask$ is 1 when the pixel value is 1, and $\mask$ becomes 0 when the pixel value is 0.95.
The soft mask allows the network to smoothly blend the residuals with the existing pixel values around the over-exposed regions.
\figref{hallucination-net} shows the design of our Hallucination-Net.


\begin{figure}
	\centering
	\includegraphics[width=1.0\linewidth]{imgs/method/hallucination_net.pdf}
	\figmargin
	\caption{
		\textbf{Architecture of Hallucination-Net.}
		We train the Hallucination-Net to predict \emph{positive} residuals and recover missing content in the over-exposed regions.
		We optimize the HDR image reconstruction loss, perceptual loss, and TV loss to generate realistic details.
	}
	\label{fig:hallucination-net}
\end{figure}


We find that the architecture of~\cite{eilertsen2017hdrcnn} may generate visible checkerboard artifacts in large over-exposed regions, as shown in~\figref{vis_checkerboard}(b).
In light of this, we replace the transposed convolutional layers in the decoder with the resize-convolution layers, i.e., nearest-neighbor upsampling followed by a $3 \times 3$ convolutional layer~\cite{odena2016deconvolution}.
The checkerboard artifacts can be significantly reduced as shown in  (see~\figref{vis_checkerboard})

\heading{Training.}
We train our Hallucination-Net by minimizing the following $\logltwo$ loss:
\begin{align}
    \halloss = \normtwo{\log(\halout) - \log(\hdr)}\,,
\end{align}
where $\hdr$ is the ground-truth HDR image.
We empirically find that training is more stable and achieves better performance when minimizing the loss in the log domain.
As the highlight regions (e.g., sun and light sources) in an HDR image typically have values with orders of magnitude larger than those of other regions, the loss is easily dominated by the errors in the highlight regions when measured in the linear domain.
Computing the loss in the log domain reduces the influence of these extremely large errors and encourages the network to restore more details in other regions.


To generate more realistic details, we further include the perceptual loss~\cite{johnson2016perceptual}:
\begin{align} \label{eq:perceptual_loss}
   \perceptualloss = \sum_{i \in \vggfeatureset} \normtwo{ \vggfeature{i}{\tmo{\halout}} - \vggfeature{i}{\tmo{\hdr}} } \,,
\end{align}
where $\vggfeature{i}{\cdot}$ denotes the feature activation at the $i$-th selected layer of the pre-trained VGG-16~\cite{VGG}.
The set $\vggfeatureset$ includes the \texttt{pool1}, \texttt{pool2}, and \texttt{pool3} layers.
As the VGG-16 is trained on non-linear RGB images, directly feeding an linear HDR image to the VGG-16 may not obtain meaningful features.
Therefore, we first apply a differentiable global tone-mapping operator~\cite{wu2018deep} to map the HDR images to a linear RGB space:
\begin{align} \label{eq:global_tmo}
    \tmo{\hdr} = \frac{\log(1 + \mu \hdr)}{\log(1 + \mu)}\,,
\end{align}
where we set $\mu = 10$.
We then compute the perceptual loss on the tone-mapped HDR images.


To improve the spatial smoothness of the predicted contents, we also minimize the total variation (TV) loss:
\begin{align} \label{eq:tv_loss}
   \tvloss = \sum_{x,y} | \partial_h \halout^{x,y}| + | \partial_v \halout^{x,y}| \,,
\end{align}
where $\partial_h$ and $\partial_v$ denote the horizontal and vertical gradient operators, respectively.


We optimize the Hallucination-Net by minimizing  $\halloss + \perceptuallossweight \perceptualloss + \tvlossweight \tvloss$.
We empirically set $\perceptuallossweight = 0.001$ and $\tvlossweight = 0.1$ in our experiments.


\heading{Discussion.}
The HDRCNN~\cite{eilertsen2017hdrcnn} generates an HDR image by a linear blending between the linear LDR image and the output of the network, i.e., $\halout = (1 - \mask) \cdot \linout + \mask \cdot \halnet{\linout}$.
The above formation is less effective as the output value may be smaller than the input in the over-exposed regions, violating the definition of saturation.
In contrast, we use a \texttt{ReLU} layer and a physically accurate formation to regularize the output of our Hallucination-Net and obtain more accurate reconstruction results.


\subsection{Joint training}
\label{sec:joint_training}

We first separately train the Dequantization-Net, Linearization-Net, and Hallucination-Net with the corresponding input and ground-truth data.
After the three networks converge, we jointly fine-tune the entire pipeline by minimizing the combination of loss functions $\totalloss$:
\begin{align} \label{eq:total_loss}
	 \deqlossweight \deqloss + \linlossweight \linloss + \crflossweight \crfloss + \hallossweight \halloss + \perceptuallossweight \perceptualloss + \tvlossweight \tvloss\,
\end{align}
where we set the weights to $\deqlossweight = 1$, $\linlossweight = 10$, $\crflossweight = 1$, $\hallossweight = 1$, $\perceptuallossweight = 0.001$, and $\tvlossweight = 0.1$.
The joint training further reduces error accumulation between the sub-networks and improve the reconstruction performance.

\subsection{Refinement}
\label{sec:refinement}

Modern camera pipeline contains significant amounts of spatially-varying operations, e.g. local tone-mapping, sharpening, chroma denoising, spatially-varying lens shading correction, and spatially-varying white balance.
So we introduce another Refinement-Net to handle whatever we could not modeled by dynamic range clipping, non-linear mapping, and quantization.

\heading{Architecture.}
Our Refinement-Net adopts the same U-Net architecture as Dequantization-Net.
Refinement-Net takes the outputs of Dequantization-Net $\deqout$, Linearization-Net $\linout$, and Hallucination-Net $\halout$ as input, and predicts a residual map.
Then we add the residual with the output of Hallucination-Net $\halout$ to produce the refined HDR image $\reout$.

\heading{Training.}
In order to model the effects of real camera pipeline, we train the Refinement-Net using self-collected exposure stacks captured by various cameras, which will be described in~\ref{sec:experiments}.
We minimize $\totalloss$ for end-to-end fine-tuning ($\deqlossweight$, $\linlossweight$, $\crflossweight$, and $\hallossweight$ are fixed as 0 as there are no stage-wise supervisions), and replace the output of Hallucination-Net $\halout$ with refined HDR image $\reout$.

\subsection{Implementation details}
\label{sec:implementation}

We implement the proposed model with TensorFlow~\cite{tensorflow}. 
We use the Adam optimizer~\cite{kingma2014adam} with a constant learning rate of $10^{-4}$ to train the Dequantization-Net, Linearization-Net, and Hallucination-Net for 500k iterations.
We then jointly fine-tune the entire model for 100k iterations by setting the learning rate to be $10^{-5}$.
The batch size is 8 when training individual networks and is 4 when jointly fine-tuning the whole model.
The entire training takes about 6 days to converge on an NVIDIA Titan Xp GPU.


We synthesize the LDR images from an HDR image dataset (described in~\secref{exp_setting}) using the camera pipeline in~\eqnref{pipeline}.
To model the sensor noise in the camera pipeline, we use a realistic noise model~\cite{foi2008practical} to add a Poisson-Gaussian noise to the clean HDR images.
The Poisson-Gaussian noise can be approximated by a heteroscedastic Gaussian with a signal-dependent variance $\realnoise{I} = I \cdot \poissonsigma + \gaussiansigma$ where $I$ is the pixel intensity.
Given a clean HDR image $\cleanhdr$, we first determine $\poissonstd$ and $\gaussianstd$ by uniformly sampling from the range of [0, 0.013] and [0, 0.005], respectively.
Then, we generate two noise maps: 
(1) a stationary noise $\gaussiannoise$ with the variance $\gaussiansigma$, 
and (2) a signal-dependent noise $\poissonnoise$ with the spatially variant variance $\cleanhdr \cdot \poissonsigma$.
Finally, a noisy HDR image $\hdr$ is generated by:
\begin{align}
	\hdr = \cleanhdr + \poissonnoise + \gaussiannoise \,,
\end{align}
which is the target ground-truth of our model.


As real-world LDR images often contain JPEG compression artifacts, we save the synthesized LDR images in a JPEG format with a quality factor randomly sampled from the range of [85, 100].
This process can be considered as a data augmentation procedure, which has been shown effective to improve the reconstruction quality on real images~\cite{eilertsen2017hdrcnn}.




==> backup_4_experiment.tex <==

\section{Experimental Results}
\label{sec:experiments}

In this section, we first describe our experimental settings and evaluation metrics.
Next, we present quantitative and qualitative comparisons with the state-of-the-art single-image HDR reconstruction algorithms.
We then analyze the contributions of individual modules to justify our design choices.
The source code, collected datasets, and our pre-trained models are available at \url{http://blinded_for_review/}.


\subsection{Experiment setups}
\label{sec:exp_setting}

As there is no standard benchmark for evaluating single-image HDR reconstruction algorithms, we construct two HDR image datasets: a synthetic dataset and a real one.
In addition, we evaluate our method on a RAW-jpeg image dataset~\cite{dang2015raise} by treating the RAW images as the HDR ground-truth.


\jiabin{Shorten the dataset description, already moved to supp}
\heading{Synthetic dataset.} 
We collect a total of 598 HDR images used in prior work~\cite{fairchild2007hdr,funt2010effect,funt2010rehabilitation,reinhard2010high,ward2006high,xiao2002high} as well as from online sources, e.g., Pfstools HDR gallery\footnote{\nolinkurl{http://pfstools.sourceforge.net/hdr_gallery.html}} and HDR-Eye\footnote{\nolinkurl{https://mmspg.epfl.ch/hdr-eye}}.
We split the dataset into 538 HDR images for training and 60 HDR images for evaluation.
All HDR images are normalized to have a mean value of 0.5 as in~\cite{endo2017drtmo}.
For each HDR image, we resize the shorter side to 512 and crop the image into two $512 \times 512$ images.



We synthesize LDR images by uniformly sampling 600 exposure times $t$ in the $\log_2$ space within $[-3, 3]$ and apply 171 different CRFs from the training set of the CRF dataset~\cite{grossberg2003space}.
In total, we generate 110,397,600 ($= 538 \times 2 \times 600 \times 171$) LDR-HDR pairs for training.
To synthesize the testing data, we sample 7 exposure times, $2^{-3}, \cdots, 2^{0}, \cdots, 2^{3}$ and apply 10 different CRFs from the test set of the CRF dataset~\cite{grossberg2003space}.
This gives a total of 8,400 ($= 60 \times 2 \times 10 \times 7$) LDR-HDR pairs for evaluation.


Our synthetic LDR images may become too dark or too bright, which are difficult for the network to generate reasonable results.
Therefore, we remove these extreme cases by the following strategy.
We first convert an LDR image to grayscale and compute the number of pixels that are within over-exposed or under-exposed regions.
The over-exposed region is defined as the pixel intensity greater than $249/255$, and the under-exposed region is defined as the pixel intensity smaller than $6/255$.
During the training stage, we exclude the LDR images which have more than $25\%$ of pixels within the over-exposed or under-exposed region.
We use the same strategy to filter out extreme cases in the test set.
After the selection, there are a total of 4,669 testing images in the synthetic dataset.

\heading{Real dataset.} 
We invite dozens of amateurs to take HDR images and instruct them to capture the scenes with multiple exposures using a steady tripod.
The LDR images are captured from 42 different cameras, including NIKON D90, NEX-5N, Canon EOS 60D, etc.
We then use Photomatix\footnote{\nolinkurl{https://www.hdrsoft.com/}} to fuse the LDR exposure stacks into HDR images, each from 5 to 20 LDR images.
In total, we have 480 HDR images and 4,893 LDR images.
70 HDR images and 919 LDR images are chosen to be testing images.
After the extreme cases selection, there are a total of 882 testing images in the real dataset.
We note that the LDR images in the synthetic dataset are \emph{synthesized} from the image formation pipeline in~\eqnref{pipeline}, while the LDR images in the real dataset are \emph{real} photos captured using different cameras with unknown pipelines.

\heading{RAISE dataset.} 
As the source HDR images in our synthetic and real datasets are generated from fusing the LDR images, there might exist some biases from the conversion tool (e.g., Photomatix).
Therefore, we also evaluate the RAISE~\cite{dang2015raise} dataset, which contains aligned RAW-TIFF image pairs.
We consider the RAW images (12 or 14 bits, depending on the capturing camera) as HDR images, which are the unprocessed signals from the camera sensors.
The TIFF images are 8-bit images processed by real camera pipelines (Nikon D90 or D7000).
We then convert the TIFF images into the JPEG format as our LDR input.
We obtain a total of 8,154 RAW-JPEG image pairs, which are more realistic images than our synthetic and real datasets.

\heading{HDR-Eye dataset.} 
We use 46 images of HDR-Eye dataset~\cite{nemoto2015visual} for testing. 
HDR-Eye dataset is composed of images taken with Sony DSC-RX100 II, Sony NEX-5N, and Sony α6000.

\heading{Evaluation metrics.} 
We adopt the HDR-VDP-2~\cite{mantiuk2011hdr} to evaluate the accuracy of HDR reconstruction. 
We first normalize both the predicted HDR and reference ground-truth HDR images with the processing steps in~\cite{marnerides2018expandnet}.
Specifically, we map the 0.1 and 99.9 percentiles of the HDR radiance in a maximum 1,000 $cd/m^2$ luminance display before calculating the HDR-VDP-2 scores.
We also evaluate the PSNR, SSIM, and perceptual score with the LPIPS metric~\cite{zhang2018perceptual} on the tone-mapped HDR images.
The LPIPS metric evaluates the perceptual distance between two images on the high-dimensional feature space of a pre-trained classification network, e.g., Squeeze-Net~\cite{Squeezenet}.

\begin{table}
    \centering
    \footnotesize
    \caption{
        \textbf{Comparisons on dequantization.}
        Our Dequantization-Net restores the missing details due to quantization and performs favorably against existing dequantization methods.
    }
    \label{tab:compare_deq}
    \begin{tabular}{l|cc}
        \toprule
        Method & PSNR & SSIM \\
        \midrule
        w/o dequantization 			& $33.86\pm6.96$ & $0.9946\pm0.0109$ \\
        \cite{daly2004decontouring} & $31.43\pm8.37$ & $0.9904\pm0.0156$ \\ 
        \cite{song2016hardware} 	& $31.49\pm8.37$ & $0.9910\pm0.0139$ \\ 
        \cite{hou2017image} 		& $33.79\pm6.72$ & $0.9936\pm0.0110$ \\
        \cite{liu2018learning} 		& $34.83\pm6.04 $ & $0.9954\pm0.0073$ \\
        Dequantization-Net (ours) 	& $\pmb{35.87\pm6.11}$ & $\pmb{0.9955\pm0.0070}$  \\ 
        \bottomrule
    \end{tabular}
\end{table}


\subsection{Ablation studies}
\label{sec:ablation}

This section evaluates the contributions of individual components in our model using the synthetic dataset.
The results in this section are tone-mapped by the same global tone-mapping operator, tone compressor, in Photomatix for better visualization and comparison.

\heading{Dequantization.} 
We consider the LDR images as the input and the image $\nonlinearhdr = \crfmapping{\clipping{\hdr}}$ synthesized from the HDR images as the ground-truth of the dequantization procedure.
We compare our Dequantization-Net with the following methods: filter-based approaches~\cite{daly2004decontouring,song2016hardware} and CNN-based models~\cite{hou2017image,liu2018learning}.
\tabref{compare_deq} shows the quantitative comparisons of dequantized images on the test set of our synthetic dataset.
As dequantization focuses on restoring low-contrast details, the differences of PSNR and SSIM between competitive methods are not significant.
However, our Dequantization-Net still performs favorably against other approaches.
\figref{vis_deq} shows the dequantization results of our model.
We provide more visual comparisons with existing dequantization methods in the supplementary material.


\begin{table}
    \centering
    \tiny
    \caption{
        \textbf{Analysis on alternatives of Linearization-Net.}
        We demonstrate the edge and histogram features and monotonically increasing constraint are effective to improve the performance of our Linearization-Net.
    }
    \label{tab:compare_lin_features}
    \begin{tabular}{cccc|cc}
        \toprule
        \multirow{2}{*}{Image} & \multirow{2}{*}{Edge} & \multirow{2}{*}{Histogram} & Monotonically & L2 error ($\downarrow$) & PSNR ($\uparrow$)
        \\
        & & & increasing & of inverse CRF & of linear image 
        \\
        \midrule
        \checkmark & & & & $2.00\pm3.15$ & $33.43\pm7.03$ \\
        \checkmark & \checkmark & & & $1.66\pm2.93$ & $34.31\pm6.94$ \\
        \checkmark & & \checkmark & & $1.61\pm3.03$ & $34.51\pm7.14$ \\
        \checkmark & \checkmark & \checkmark & & $1.58\pm2.73$ & $34.53\pm6.83$ \\ 
        \checkmark & \checkmark & \checkmark & \checkmark & $\pmb{1.56\pm2.52}$ & $\pmb{34.64\pm6.73}$ \\ 
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}
    \centering
    \footnotesize
    \caption{
        \textbf{Comparison on linearization.}
        * represents that the model is re-trained on our training data.
        The proposed Linearization-Net reconstructs more accurate inverse CRFs than existing approaches.
    }
    \label{tab:compare_lin}
    \begin{tabular}{l|cc}
        \toprule
        \multirow{2}{*}{Method} & L2 error ($\downarrow$) & PSNR ($\uparrow$)
        \\
         & of inverse CRF & of linear image 
        \\
        \midrule
        Pre-defined $x^2$~\cite{eilertsen2017hdrcnn} & $11.64\pm12.47$ & $24.81\pm6.47$ \\
        Pre-defined $x^{2.2}$ & \enspace$9.06\pm10.74$ & $25.82\pm6.04$ \\
        Average inverse CRF & $7.36\pm7.03$ & $25.24\pm4.82$ \\
        CRF-Net~\cite{li2017crfnet} & $4.23\pm4.37$ & $30.61\pm6.82$ \\ 
        CRF-Net*~\cite{li2017crfnet} & $2.71\pm4.10$ & $32.84\pm6.85$ \\ 
        Linearization-Net (ours) & $\pmb{1.56\pm2.52}$ & $\pmb{34.64\pm6.73}$ \\ 
        \bottomrule
    \end{tabular}
\end{table}


\heading{Linearization.} 
Our Linearization-Net takes as input the non-linear LDR image, Sobel filter responses, and histogram features to estimate an inverse CRF.
To validate the effectiveness of these factors, we train our Linearization-Net with different combinations of the edge and histogram features.
\tabref{compare_lin_features} shows the reconstruction error of the inverse CRF and the PSNR between the output of our Linearization-Net and the corresponding ground-truth image $\cliphdr = \clipping{\hdr}$.
The edge and histogram features help predict more accurate inverse CRFs.
The monotonically increasing constraint further boosts the reconstruction performance on both the inverse CRFs and the linear images.


Next, we compare the proposed Linearization-Net with existing approaches, including pre-defined curves $\invcrf = x^2$ and $\invcrf = x^{2.2}$, the average inverse CRF in the CRF dataset~\cite{grossberg2003space}, and the CRF-Net~\cite{li2017crfnet}.
We also re-train the CRF-Net on our training data for fair comparisons (marked with *).
As shown in~\tabref{compare_lin}, the proposed Linearization-Net obtains the lowest reconstruction error of inverse CRFs as well as the highest PSNR values.
We provide visualization of the reconstructed inverse CRFs and linear images in the supplementary material.


\begin{table}
    \centering
    \scriptsize
    \caption{
        \textbf{Analysis on alternatives of Hallucination-Net.}
        With the positive residual learning, the model predicts physically accurate values within the over-exposed regions.
        The resize convolution reduces the checkerboard artifacts, while the perceptual loss helps generate realistic details.
    }
    \label{tab:compare_hal}
    \begin{tabular}{ccc|c}
	    \toprule
	    Positive residual & Resize convolution & Perceptual loss & HDR-VDP-2 \\
		\midrule
	    & & & $63.60\pm15.32$ \\
	    \checkmark & & &$64.79\pm15.89$ \\
	    \checkmark & \checkmark & & $64.52\pm16.05$ \\  
	    \checkmark & \checkmark & \checkmark & \pmb{$66.31\pm15.82$} \\
	    \bottomrule
    \end{tabular}
    \tabmargin
\end{table}

\heading{Hallucination.} 
Our Hallucination-Net takes as input an LDR image $\cliphdr = \clipping{\hdr}$ and reconstructs an HDR image $\hdr$.
We start with the architecture of Eilertsen~\etal~\cite{eilertsen2017hdrcnn}, which does not enforce the predicted residuals being positive.
As shown in~\tabref{compare_hal}, our model with a simple \texttt{ReLU} layer to predict positive residuals can improve the performance by 1.19 HDR-VDP-2 scores.
By replacing the transposed convolution with the resize convolution in the decoder, our model effectively reduces the checkerboard artifacts as shown in~\figref{vis_checkerboard}.
Furthermore, introducing the perceptual loss for training not only improves the HDR-VDP-2 scores but also helps the model to predict more realistic details.
We provide visual comparisons in the supplementary material.


\begin{table}[t]
    \caption{
        \textbf{Quantitative comparison on HDR images with existing methods.} %
        * represents that the model is re-trained on our synthetic training data and + is fine-tuned on both synthetic and real training data. \textcolor{red}{\pmb{Red}} text indicates the best and \textcolor{blue}{\underline{blue}} text indicates the best performing state-of-the-art method.
    }
    \label{tab:compare_stoa_hdrvdp}
    \centering
    \tiny
    \tabmargin
    \begin{tabular}{l|c|cccc}
        \toprule
        Method & Training dataset & Synthetic & Real & RAISE & HDR-Eye \\
        \midrule
        AEO~\cite{akyuz2007hdr} & - & $54.67\pm9.22$ & $48.47\pm8.27$ & $56.54\pm4.00$ & $49.20\pm5.81$ \\
        HPEO~\cite{huo2014physiological} & - & $51.08\pm8.10$ & $46.29\pm6.70$ & $55.16\pm5.40$ & $44.12\pm4.75$ \\
        KOEO~\cite{kovaleski2014high} & - & $54.93\pm7.56$ & $50.19\pm7.42$ & $54.33\pm4.72$ & $49.62\pm6.06$ \\
        MEO~\cite{masia2017dynamic} & - & $55.02\pm9.07$ & $48.50\pm8.33$ & $56.30\pm3.72$ & $49.28\pm6.09$ \\
        HDRCNN~\cite{eilertsen2017hdrcnn} & pre-trained & $56.94\pm7.99$ & $49.74\pm7.82$ & $57.08\pm3.77$ & $50.80\pm5.79$ \\
        HDRCNN*~\cite{eilertsen2017hdrcnn} & synthetic & \textcolor{blue}{\underline{$58.72\pm6.57$}} & $50.02\pm6.96$ & $54.72\pm3.84$ & $50.57\pm5.07$ \\
        HDRCNN+~\cite{eilertsen2017hdrcnn} & synthetic+real & $55.51\pm6.64$ & \textcolor{blue}{\underline{$51.38\pm7.17$}} & $56.51\pm4.33$ & $51.08\pm5.84$ \\
        DrTMO~\cite{endo2017drtmo} & pre-trained & $57.15\pm6.95$ & $50.55\pm7.25$ & $57.69\pm4.08$ & $51.80\pm5.93$ \\
        DrTMO*~\cite{endo2017drtmo} & synthetic & $56.74\pm7.54$ & $50.20\pm7.57$ & $57.65\pm3.62$ & \textcolor{blue}{\underline{$51.47\pm5.88$}}\\
        DrTMO+~\cite{endo2017drtmo} & synthetic+real & $56.41\pm7.20$ & $50.77\pm7.78$ & \textcolor{blue}{\underline{$57.92\pm3.69$}} & $51.26\pm5.94$ \\
        ExpandNet~\cite{marnerides2018expandnet} & pre-trained & $53.55\pm4.98$ & $48.67\pm6.46$ & $54.62\pm1.99$ & $50.43\pm5.49$ \\
        Deep chain HDRI~\cite{lee2018deepchain} & pre-trained & - & - & - & $49.80\pm5.97$ \\
        Deep recursive HDRI~\cite{lee2018deep} & pre-trained & - & - & - & $48.85\pm4.91$ \\
        Ours* & synthetic & \textcolor{red}{$\pmb{60.11\pm6.10}$} & $51.59\pm7.42$ & $58.80\pm3.91$ & $52.66\pm5.64$\\
        Ours+ & synthetic+real & $59.52\pm6.02$ & \textcolor{red}{\pmb{$53.16\pm7.19$}} & \textcolor{red}{\pmb{$59.21\pm3.68$}} & \textcolor{red}{\pmb{$53.16\pm5.92$}} \\
        \bottomrule
    \end{tabular}
    \tabmargin
\end{table}


\input{figures/fig_visual_stoa}


\subsection{Comparisons with state-of-the-art methods}
\label{sec:compare_SOTA}

We compare the proposed method with four conventional single-image HDR reconstruction methods: Aky{\"u}z~\etal~\cite{akyuz2007hdr}, Huo~\etal~\cite{huo2014physiological}, Kovaleski and Oliveira~\cite{kovaleski2014high}, and Masia~\etal~\cite{masia2017dynamic}, and five recent CNN-based approaches: HDRCNN~\cite{eilertsen2017hdrcnn}, DrTMO~\cite{endo2017drtmo}, ExpandNet~\cite{marnerides2018expandnet}, Deep chain HDRI~\cite{lee2018deepchain}, and Deep recursive HDRI~\cite{lee2018deep}. 
For fair comparisons, we re-train the HDRCNN and DrTMO models using our training data. Both methods trained using syntheitc dataset are denoted by HDRCNN* and DrTMO*, and trained using both synthetic and real dataset are denoted by HDRCNN+ and DrTMO+.
As the ExpandNet does not provide the code for training, we only compare with their pre-trained model.
Deep chain HDRI and Deep recursive HDRI does not provide pre-trained model, so we compare with the number reported by their paper.

\heading{Quantitative comparisons.}
\tabref{compare_stoa_hdrvdp} shows the average HDR-VDP-2 scores on the synthetic, real, RAISE, and HDR-Eye datasets.
In general, CNN-based approaches~\cite{eilertsen2017hdrcnn,endo2017drtmo,marnerides2018expandnet} perform better than conventional methods~\cite{akyuz2007hdr,huo2014physiological,kovaleski2014high,masia2017dynamic}.
Among the CNN-based models, the proposed method performs favorably against the state-of-the-art methods on all four datasets.
After fine-tuning using both synthetic and real dataset, the performance of our model is further improved by 1.57 on the real, 0.41 on the RAICE, and 0.5 on the HDR-Eye datasets, respectively.


\heading{Visual comparisons.} 
\figref{visual_synthetic}, \ref{fig:visual_real}, and \ref{fig:visual_hdreye} show several challenging examples on the synthetic, real, and HDR-Eye datasets, where a large portion of details are missing due to sensor saturation in the over-exposed areas and quantization in the under-exposed areas. 
Compared to the state-of-the-art algorithms, our method is capable of restoring missing details washed away from sunlight or hidden by dim light, filling in plausible contents, and generating natural-looking images without visual artifacts. 


\figref{visual_sota} compares the proposed model with existing methods on an example provided in~\cite{endo2017drtmo} and a real image captured using Apple iPhone X provided by DxOMark~\cite{DxO}.
In general, the HDRCNN~\cite{eilertsen2017hdrcnn} tends to produce over-bright results and often suffers from noise in the under-exposed regions.
The DrTMO~\cite{endo2017drtmo} cannot handle the over-exposed regions well as shown in the sky of \ref{fig:visual_real} and \figref{visual_sota}.
The ExpandNet~\cite{marnerides2018expandnet} often fails to restore faithful details.

We provide more visual comparisons with the CNN-based approaches~\cite{eilertsen2017hdrcnn,endo2017drtmo,marnerides2018expandnet} as well as conventional methods~\cite{akyuz2007hdr,huo2014physiological,kovaleski2014high,masia2017dynamic} in the supplementary material.



\heading{Human subject study.}
We conduct a user study to evaluate the human preference on HDR images. 
We adopt the paired comparison~\cite{Rubinstein-TOG-2010,Lai-CVPR-2016}, where the user is asked to select a preferred image from a pair of images in each comparison.
We design the user study with the following two settings:
(1) \textit{With-reference test}: We show the input LDR as well as the ground-truth HDR images as reference.
This test evaluates the faithfulness of the reconstructed HDR image to the ground-truth.
(2) \textit{No-reference test}: The input LDR and ground-truth HDR images are not shown for reference.
This test mainly compares the visual quality of two reconstructed HDR images.

We evaluate all 80 HDR images in the real dataset.
We compare the proposed method with the HDRCNN~\cite{eilertsen2017hdrcnn}, DrTMO~\cite{endo2017drtmo}, and ExpandNet~\cite{marnerides2018expandnet}.
We ask each participant to compare 30 pairs of images and collect the votes from a total of 200 unique participants.
\figref{user_study} reports the percentages of the head-to-head comparisons in which users prefer our method over the HDRCNN, DrTMO, and ExpandNet in both with-reference and no-reference tests.
Overall, there are $70\%$ and $69\%$ of users prefer our results in the with-reference and no-reference tests, respectively.
The with-reference test shows that our model generates faithful results that are close to the ground-truth.
In the no-reference test, users may focus more on comparing the details and visual artifacts between two results.
Therefore, the no-reference test demonstrates that our reconstructed results are more visually pleasing with fewer visual artifacts.
Both user studies show that the proposed method performs well to human subjective perception.


\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{imgs/userstudy.pdf}
    \figmargin
\caption{
    \textbf{Results of user study.}
    The with-reference test shows that our model generates faithful results that are similar to ground-truth.
    The no-reference test demonstrates that our reconstructed results are more visually pleasing and contain fewer artifacts.
    }
\label{fig:user_study}
\end{figure}







